RecallWorld: Episodic Memory for Persistent Embodied Video World Models

Video world models generate plausible novel views but often lack persistent memory, failing to preserve a place's geometry and appearance when an agent revisits a scene. A central challenge is how previous views should be effectively used for creating memory. Reconstructing them independently underutilizes geometric constraints between nearby views, while repeatedly reconstructing a growing history can propagate later prediction errors into earlier geometry. We introduce RecallWorld, a persistent embodied video world model that jointly reconstructs short multi-view episodes into Scenelets while keeping geometry independent across episodes. Starting from a single source image, camera-aware ray lifting places perspective and native fisheye images in a common world frame, retaining wide-field content for perspective generation. Each generated segment extends the Scenelet memory and conditions subsequent generation. Coverage-based retrieval selects complementary Scenelets from the full history, while target-view visibility is resolved geometrically before appearance fusion, providing consistent memory conditioning for guiding subsequent generation. Across four datasets, RecallWorld improves revisit PSNR over the strongest evaluated baseline by 2.6 dB on partial revisits and 3.9 dB on full cycles, demonstrating substantially stronger preservation of scene identity across exploration and return.

==> figures/fisheye/layout.tex <==
% Only the method label changes; original scientific image streams are retained.
\begingroup%
\begin{tikzpicture}[x=1bp,y=-1bp,
  every node/.style={inner sep=0pt,outer sep=0pt}]
\path[use as bounding box] (0,0) rectangle (291,77);
\node[anchor=north west] at (0,0)
  {\includegraphics[width=291bp]{figures/fisheye/label-base.pdf}};
\node[font=\rmfamily\fontsize{8}{9}\selectfont\bfseries,
  text=navworldred] at (233.542,6.493)
  {\navworldfisheye{} (OURS)};
\end{tikzpicture}%
\endgroup%

